O3D: Offline Data-driven Discovery and Distillation for Sequential Decision-Making with Large Language Models

Recent advancements in large language models (LLMs) have exhibited promising performance in solving sequential decision-making problems. By imitating few-shot examples provided in the prompts (i.e., in-context learning), an LLM agent can interact with an external environment and complete given tasks without additional training. However, such few-shot examples are often insufficient to generate high-quality solutions for complex and long-horizon tasks, while the limited context length cannot consume larger-scale demonstrations with long interaction horizons. To this end, we propose an offline learning framework that utilizes offline data at scale (e.g, logs of human interactions) to improve LLM-powered policies without finetuning. The proposed method O3D (Offline Data-driven Discovery and Distillation) automatically discovers reusable skills and distills generalizable knowledge across multiple tasks based on offline interaction data, advancing the capability of solving downstream tasks. Empirical results under two interactive decision-making benchmarks (ALFWorld and WebShop) verify that O3D can notably enhance the decision-making capabilities of LLMs through the offline discovery and distillation process, and consistently outperform baselines across various LLMs.

==> algos_backup.tex <==
% \begin{figure}[t]
% \vspace{-2em}

\begin{algorithm}
\SetAlgoNoLine
\newcommand\mycommfont[1]{\footnotesize\ttfamily\textcolor{gray}{#1}}
\SetCommentSty{mycommfont}
    \caption{Offline Policy Improvement with \llmpolname}
    \label{alg:llmpolalg}
    \textbf{Input:} Pre-trained LLM, offline dataset $\data$, success score threshold $R_S$, failure score threshold $R_F$, batch size $\bs$\\
    \textbf{Output:} \llmpolname $\llmpolicy$\\
    \tcp{Stage 1: skill discovery and data segmentation}
    Initialize sets of skills $\skills=\emptyset$\\
    Select success trajectories $\data_S \leftarrow \data(R \geq R_S)$, failure trajectories $\data_F \leftarrow \data(R \leq R_F)$\\
    \Repeat{No new skill can be discovered}{
        Sample $N$ trajectories $d_S \sim \data_S$\\
        Distill skills $\skills \leftarrow LLM(\skills, d_S; \textcolor{blue}{\mathsf{DiscoverPrompt}})$\\
    }
    Segment trajectories of $\data_S$ and $\data_F$ based on skills, obtain $\data^{\skill_k}_S$ and $\data^{\skill_k}_F$ for each $\skill_k \in \skills$\\
    \tcp{Stage 2: skill-conditioned policy improvement}
    \For{$\skill_k \in \skills$}{
        Initialize sets of primitives $\prims^{\skill_k}$ and tips $\tips^{\skill_k}$ associated with skill $\skill_k$: \\
        \Repeat{No new primitive can be discovered}{
            Sample $N$ trajectories $d^{\skill_k}_S \sim \data^{\skill_k}_S$\\
            Distill primitives $\prims\leftarrow LLM(\prims^{\skill_k}, d^{\skill_k}_S; \textcolor{blue}{\mathsf{DiscoverPrompt}})$\\
        }
        \Repeat{No new tip can be distilled}{
            Sample success-failure pairs of trajectories: $\{(d^{\skill_k}_S,d^{\skill_k}_F) \sim (\data^{\skill_k}_S, \data^{\skill_k}_F)$\\
            Distill policy improvement knowledge $\tips^{\skill_k} \leftarrow LLM(\tips^{\skill_k}, (d^{\skill_k}_S,d^{\skill_k}_F); \textcolor{red}{\mathsf{DistillPrompt}})$\\
        }
    }
    \tcp{Stage 3: policy regularization and composition}
    For each skill $\skill_k \in \skills$, obtain skill-based LLM policy $\llmpolicy^{\skill_k}$ with primitives $\prims^{\skill_k}$, tips $\tips^{\skill_k}$, and sampled success examples $d^{\skill_k}_S \sim \data^{\skill_k}_S$.\\
    Use $\data_S$ to prompt the main policy $\llmpolicy$ to interact with the environment by calling skills. \\
\end{algorithm}


\begin{algorithm}
\SetAlgoNoLine
\newcommand\mycommfont[1]{\footnotesize\ttfamily\textcolor{gray}{#1}}
\SetCommentSty{mycommfont}
    \caption{Offline Policy Improvement with \codepolname}
    \label{alg:codepolalg}
    \textbf{Input:} Pre-trained LLM, offline dataset $\data$, success score threshold $R_S$, failure score threshold $R_F$, batch size $\bs$\\
    \textbf{Output:} \codepolname $\codepolicy$\\
    \tcp{Stage 1: skill discovery and data segmentation}
    Initialize sets of skills $\skills=\emptyset$\\
    Select success trajectories $\data_S \leftarrow \data(R \geq R_S)$, failure trajectories $\data_F \leftarrow \data(R \leq R_F)$\\
    \Repeat{No new skill can be discovered}{
        Sample $N$ trajectories $d_S \sim \data_S$\\
        Distill skills $\skills \leftarrow LLM(\skills, d_S; \textcolor{blue}{\mathsf{DiscoverPrompt}})$\\
    }
    Segment trajectories of $\data_S$ and $\data_F$ based on skills, obtain $\data^{\skill_k}_S$ and $\data^{\skill_k}_F$ for each $\skill_k \in \skills$\\
    \tcp{Stage 2: skill-conditioned policy improvement}
    \For{$\skill_k \in \skills$}{
        Initialize sets of primitives $\prims^{\skill_k}$ and tips $\tips^{\skill_k}$ associated with skill $\skill_k$: \\
        \Repeat{No new primitive can be discovered}{
            Sample $N$ trajectories $d^{\skill_k}_S \sim \data^{\skill_k}_S$\\
            Distill primitives $\prims\leftarrow LLM(\prims^{\skill_k}, d^{\skill_k}_S; \textcolor{blue}{\mathsf{DiscoverPrompt}})$\\
        }
        \Repeat{No new tip can be distilled}{
            Sample success-failure pairs of trajectories: $\{(d^{\skill_k}_S,d^{\skill_k}_F) \sim (\data^{\skill_k}_S, \data^{\skill_k}_F)$\\
            Distill policy improvement knowledge $\tips^{\skill_k} \leftarrow LLM(\tips^{\skill_k}, (d^{\skill_k}_S,d^{\skill_k}_F); \textcolor{red}{\mathsf{DistillPrompt}})$\\
        }
    }
    \tcp{Stage 3: policy regularization and composition}
    For each skill $\skill_k \in \skills$, obtain skill-based LLM policy $\llmpolicy^{\skill_k}$ with primitives $\prims^{\skill_k}$, tips $\tips^{\skill_k}$, and sampled success examples $d^{\skill_k}_S \sim \data^{\skill_k}_S$.\\
    Use $\data_S$ to prompt the main policy $\llmpolicy$ to interact with the environment by calling skills. \\
\end{algorithm}




% \begin{algorithm}[H]
% \caption{Offline Policy Optimization with \llmpolname}
% \label{alg:llmpolalg}
% \SetAlgoLined
%     \textbf{Input:} Pre-trained LLM with weights $\pretpara$, dataset $\data$, success score threshold $R_S$, failure score threshold $R_F$, batch size $\bs$\\
%     \textbf{Output:} \llmpolname $\llmpolicy$\\
%     Initialize sets of primitives $\prims=\emptyset$\\
%     Select success trajectories $\data_S \leftarrow \data(R \geq R_S)$, failure trajectories $\data_F \leftarrow \data(R \leq R_F)$\\
%     \Repeat{Converge}{
%         Sample trajectories $\{d_i\}_{i=1}^\bs \sim \data_S$\\
%         Distill primitives $\prims\leftarrow LLM(\prims, \mathsf{UpdatePrompt})$\\
%     }
%     Initialize tips set $\tips=\emptyset$\\
%     \Repeat{Converge}{
%         Sample success-failure pairs of trajectories: $\{(d_S,d_F)_i\}_{i=1}^\bs \sim (\data_S, \data_F)$\\
%         Distill policy improvement knowledge $\tips \leftarrow LLM(\tips, \mathsf{ContrastUpdatePrompt})$\\
%     }
%     Format the online-learning prompt $\prompara := \mathsf{OnlinePrompt}(\prims, \tips, \mathsf{Examples})$\\
%     \textbf{Return} $LLM(\prompara, \pretpara)$\\
% \end{algorithm}
% % \vspace{-1.5em}
% % \end{figure}


% \begin{algorithm}[H]
% \caption{Offline Policy Optimization with \codepolname}
% \label{alg:codepolalg}
%     \textbf{Input:} Pre-trained LLM with weights $\pretpara$, dataset $\data$, success score threshold $R_S$, failure score threshold $R_F$, batch size $\bs$\\
%     \textbf{Output:} \codepolname $\codepolicy$\\ 
% \end{algorithm}

% \begin{algorithm}
%     \caption{Hierarchical Policy Optimization}
%     \label{alg:hier}
%     \textbf{Input:} Pre-trained LLM with weights $\pretpara$, dataset $\data$, success score threshold $R_S$, failure score threshold $R_F$, batch size $\bs$\\
%     \textbf{Output:} High-level policy $\pi^H$ and low-level skill-based policies $\{\pi^L_k\}$\\
%     Initialize sets of skills $\skills=\emptyset$\\
%     Select success trajectories $\data_S \leftarrow \data(R \geq R_S)$\\
%     \Repeat{Converge}{
%         Sample trajectories $\{d_i\}_{i=1}^\bs \sim \data_S$\\
%         Distill skills $\skills \leftarrow LLM(\skills, \mathsf{UpdatePrompt})$\\
%     }
%     Segment trajectories of $\data$ based on skills, obtain $\data^{\skill_k}$ for each $\skill_k \in \skills$\\
%     \For{$\skill_k \in \skills$}{
%         $\pi^L_k \leftarrow$ \Cref{alg:llmpolalg} (\llmpolname) or \Cref{alg:codepolalg} (\codepolname) with dataset $\data^{\skill_k}$ and other hyper-parameters\\
%     }
% \end{algorithm}

==> plots/barchart.tex <==
\begin{tikzpicture}

\definecolor{darkgray176}{RGB}{176,176,176}
\definecolor{darkorange25512714}{RGB}{255,127,14}
\definecolor{forestgreen4416044}{RGB}{44,160,44}
\definecolor{lightgray204}{RGB}{204,204,204}
\definecolor{steelblue31119180}{RGB}{31,119,180}

\begin{groupplot}[group style={group size=7 by 2}]
\nextgroupplot[
tick align=outside,
tick pos=left,
x grid style={darkgray176},
xlabel={Put},
xmin=-0.0325, xmax=0.1325,
xtick style={color=black},
y grid style={darkgray176},
ylabel={# of Tasks},
ymin=0, ymax=26,
ytick style={color=black}
]
\draw[draw=none,fill=steelblue31119180] (axis cs:-0.025,0) rectangle (axis cs:0.025,19);
\addlegendimage{ybar,ybar legend,draw=none,fill=steelblue31119180}
\addlegendentry{O3D-S}

\draw[draw=none,fill=darkorange25512714] (axis cs:0.025,0) rectangle (axis cs:0.075,18);
\addlegendimage{ybar,ybar legend,draw=none,fill=darkorange25512714}
\addlegendentry{O3D-P}

\draw[draw=none,fill=forestgreen4416044] (axis cs:0.075,0) rectangle (axis cs:0.125,15);
\addlegendimage{ybar,ybar legend,draw=none,fill=forestgreen4416044}
\addlegendentry{O3D-DK}

\addplot [semithick, black, dash pattern=on 1pt off 3pt on 3pt off 3pt]
table {%
-0.0325 16
0.1325 16
};
\addplot [semithick, red, dashed]
table {%
-0.0325 22
0.1325 22
};

\nextgroupplot[
tick align=outside,
tick pos=left,
x grid style={darkgray176},
xlabel={Clean},
xmin=-0.0325, xmax=0.1325,
xtick style={color=black},
y grid style={darkgray176},
ymin=0, ymax=33,
ytick style={color=black}
]
\draw[draw=none,fill=steelblue31119180] (axis cs:-0.025,0) rectangle (axis cs:0.025,29);
\draw[draw=none,fill=darkorange25512714] (axis cs:0.025,0) rectangle (axis cs:0.075,27);
\draw[draw=none,fill=forestgreen4416044] (axis cs:0.075,0) rectangle (axis cs:0.125,23);
\addplot [semithick, black, dash pattern=on 1pt off 3pt on 3pt off 3pt]
table {%
-0.0325 23
0.1325 23
};
\addplot [semithick, red, dashed]
table {%
-0.0325 31
0.1325 31
};

\nextgroupplot[
tick align=outside,
tick pos=left,
x grid style={darkgray176},
xlabel={Heat},
xmin=-0.0325, xmax=0.1325,
xtick style={color=black},
y grid style={darkgray176},
ymin=0, ymax=25,
ytick style={color=black}
]
\draw[draw=none,fill=steelblue31119180] (axis cs:-0.025,0) rectangle (axis cs:0.025,20);
\draw[draw=none,fill=darkorange25512714] (axis cs:0.025,0) rectangle (axis cs:0.075,22);
\draw[draw=none,fill=forestgreen4416044] (axis cs:0.075,0) rectangle (axis cs:0.125,20);
\addplot [semithick, black, dash pattern=on 1pt off 3pt on 3pt off 3pt]
table {%
-0.0325 17
0.1325 17
};
\addplot [semithick, red, dashed]
table {%
-0.0325 22
0.1325 22
};

\nextgroupplot[
tick align=outside,
tick pos=left,
x grid style={darkgray176},
xlabel={Cool},
xmin=-0.0325, xmax=0.1325,
xtick style={color=black},
y grid style={darkgray176},
ymin=0, ymax=23,
ytick style={color=black}
]
\draw[draw=none,fill=steelblue31119180] (axis cs:-0.025,0) rectangle (axis cs:0.025,19);
\draw[draw=none,fill=darkorange25512714] (axis cs:0.025,0) rectangle (axis cs:0.075,20);
\draw[draw=none,fill=forestgreen4416044] (axis cs:0.075,0) rectangle (axis cs:0.125,15);
\addplot [semithick, black, dash pattern=on 1pt off 3pt on 3pt off 3pt]
table {%
-0.0325 14
0.1325 14
};
\addplot [semithick, red, dashed]
table {%
-0.0325 20
0.1325 20
};

\nextgroupplot[
tick align=outside,
tick pos=left,
x grid style={darkgray176},
xlabel={Look},
xmin=-0.0325, xmax=0.1325,
xtick style={color=black},
y grid style={darkgray176},
ymin=0, ymax=20,
ytick style={color=black}
]
\draw[draw=none,fill=steelblue31119180] (axis cs:-0.025,0) rectangle (axis cs:0.025,18);
\draw[draw=none,fill=darkorange25512714] (axis cs:0.025,0) rectangle (axis cs:0.075,18);
\draw[draw=none,fill=forestgreen4416044] (axis cs:0.075,0) rectangle (axis cs:0.125,17);
\addplot [semithick, black, dash pattern=on 1pt off 3pt on 3pt off 3pt]
table {%
-0.0325 18
0.1325 18
};
\addplot [semithick, red, dashed]
table {%
-0.0325 18
0.1325 18
};

\nextgroupplot[
tick align=outside,
tick pos=left,
x grid style={darkgray176},
xlabel={Pick 2},
xmin=-0.0325, xmax=0.1325,
xtick style={color=black},
y grid style={darkgray176},
ymin=0, ymax=19,
ytick style={color=black}
]
\draw[draw=none,fill=steelblue31119180] (axis cs:-0.025,0) rectangle (axis cs:0.025,6);
\draw[draw=none,fill=darkorange25512714] (axis cs:0.025,0) rectangle (axis cs:0.075,11);
\draw[draw=none,fill=forestgreen4416044] (axis cs:0.075,0) rectangle (axis cs:0.125,8);
\addplot [semithick, black, dash pattern=on 1pt off 3pt on 3pt off 3pt]
table {%
-0.0325 8
0.1325 8
};
\addplot [semithick, red, dashed]
table {%
-0.0325 9
0.1325 9
};

\nextgroupplot[
tick align=outside,
tick pos=left,
title={GPT-4},
x grid style={darkgray176},
xlabel={SR},
xmin=-0.0325, xmax=0.1325,
xtick style={color=black},
y grid style={darkgray176},
ymin=0, ymax=1.05,
ytick style={color=black}
]
\draw[draw=none,fill=steelblue31119180] (axis cs:-0.025,0) rectangle (axis cs:0.025,0.83);
\draw[draw=none,fill=darkorange25512714] (axis cs:0.025,0) rectangle (axis cs:0.075,0.87);
\draw[draw=none,fill=forestgreen4416044] (axis cs:0.075,0) rectangle (axis cs:0.125,0.73);
\addplot [semithick, black, dash pattern=on 1pt off 3pt on 3pt off 3pt]
table {%
-0.0325000000000002 0.72
0.1325 0.72
};
\addplot [semithick, red, dashed]
table {%
-0.0325000000000002 0.91
0.1325 0.91
};

\nextgroupplot[
tick align=outside,
tick pos=left,
x grid style={darkgray176},
xlabel={Put},
xmin=-0.0325, xmax=0.1325,
xtick style={color=black},
y grid style={darkgray176},
ylabel={# of Tasks},
ymin=0, ymax=26,
ytick style={color=black}
]
\draw[draw=none,fill=steelblue31119180] (axis cs:-0.025,0) rectangle (axis cs:0.025,11);
\draw[draw=none,fill=darkorange25512714] (axis cs:0.025,0) rectangle (axis cs:0.075,10);
\draw[draw=none,fill=forestgreen4416044] (axis cs:0.075,0) rectangle (axis cs:0.125,4);
\addplot [semithick, black, dash pattern=on 1pt off 3pt on 3pt off 3pt]
table {%
-0.0325 3
0.1325 3
};
\addplot [semithick, red, dashed]
table {%
-0.0325 17
0.1325 17
};

\nextgroupplot[
tick align=outside,
tick pos=left,
x grid style={darkgray176},
xlabel={Clean},
xmin=-0.0325, xmax=0.1325,
xtick style={color=black},
y grid style={darkgray176},
ymin=0, ymax=33,
ytick style={color=black}
]
\draw[draw=none,fill=steelblue31119180] (axis cs:-0.025,0) rectangle (axis cs:0.025,15);
\draw[draw=none,fill=darkorange25512714] (axis cs:0.025,0) rectangle (axis cs:0.075,7);
\draw[draw=none,fill=forestgreen4416044] (axis cs:0.075,0) rectangle (axis cs:0.125,3);
\addplot [semithick, black, dash pattern=on 1pt off 3pt on 3pt off 3pt]
table {%
-0.0325 3
0.1325 3
};
\addplot [semithick, red, dashed]
table {%
-0.0325 11
0.1325 11
};

\nextgroupplot[
tick align=outside,
tick pos=left,
x grid style={darkgray176},
xlabel={Heat},
xmin=-0.0325, xmax=0.1325,
xtick style={color=black},
y grid style={darkgray176},
ymin=0, ymax=25,
ytick style={color=black}
]
\draw[draw=none,fill=steelblue31119180] (axis cs:-0.025,0) rectangle (axis cs:0.025,4);
\draw[draw=none,fill=darkorange25512714] (axis cs:0.025,0) rectangle (axis cs:0.075,0);
\draw[draw=none,fill=forestgreen4416044] (axis cs:0.075,0) rectangle (axis cs:0.125,2);
\addplot [semithick, black, dash pattern=on 1pt off 3pt on 3pt off 3pt]
table {%
-0.0325 -8.88178419700125e-16
0.1325 -8.88178419700125e-16
};
\addplot [semithick, red, dashed]
table {%
-0.0325 0.999999999999999
0.1325 0.999999999999999
};

\nextgroupplot[
tick align=outside,
tick pos=left,
x grid style={darkgray176},
xlabel={Cool},
xmin=-0.0325, xmax=0.1325,
xtick style={color=black},
y grid style={darkgray176},
ymin=0, ymax=23,
ytick style={color=black}
]
\draw[draw=none,fill=steelblue31119180] (axis cs:-0.025,0) rectangle (axis cs:0.025,12);
\draw[draw=none,fill=darkorange25512714] (axis cs:0.025,0) rectangle (axis cs:0.075,6);
\draw[draw=none,fill=forestgreen4416044] (axis cs:0.075,0) rectangle (axis cs:0.125,4);
\addplot [semithick, black, dash pattern=on 1pt off 3pt on 3pt off 3pt]
table {%
-0.0325 0
0.1325 0
};
\addplot [semithick, red, dashed]
table {%
-0.0325 14
0.1325 14
};

\nextgroupplot[
tick align=outside,
tick pos=left,
x grid style={darkgray176},
xlabel={Look},
xmin=-0.0325, xmax=0.1325,
xtick style={color=black},
y grid style={darkgray176},
ymin=0, ymax=20,
ytick style={color=black}
]
\draw[draw=none,fill=steelblue31119180] (axis cs:-0.025,0) rectangle (axis cs:0.025,5);
\draw[draw=none,fill=darkorange25512714] (axis cs:0.025,0) rectangle (axis cs:0.075,4);
\draw[draw=none,fill=forestgreen4416044] (axis cs:0.075,0) rectangle (axis cs:0.125,4);
\addplot [semithick, black, dash pattern=on 1pt off 3pt on 3pt off 3pt]
table {%
-0.0325 3
0.1325 3
};
\addplot [semithick, red, dashed]
table {%
-0.0325 8
0.1325 8
};

\nextgroupplot[
tick align=outside,
tick pos=left,
x grid style={darkgray176},
xlabel={Pick 2},
xmin=-0.0325, xmax=0.1325,
xtick style={color=black},
y grid style={darkgray176},
ymin=0, ymax=19,
ytick style={color=black}
]
\draw[draw=none,fill=steelblue31119180] (axis cs:-0.025,0) rectangle (axis cs:0.025,2);
\draw[draw=none,fill=darkorange25512714] (axis cs:0.025,0) rectangle (axis cs:0.075,3);
\draw[draw=none,fill=forestgreen4416044] (axis cs:0.075,0) rectangle (axis cs:0.125,0);
\addplot [semithick, black, dash pattern=on 1pt off 3pt on 3pt off 3pt]
table {%
-0.0325 -8.88178419700125e-16
0.1325 -8.88178419700125e-16
};
\addplot [semithick, red, dashed]
table {%
-0.0325 4
0.1325 4
};

\nextgroupplot[
tick align=outside,
tick pos=left,
title={GPT-3.5},
x grid style={darkgray176},
xlabel={SR},
xmin=-0.0325, xmax=0.1325,
xtick style={color=black},
y grid style={darkgray176},
ymin=0, ymax=1.05,
ytick style={color=black}
]
\draw[draw=none,fill=steelblue31119180] (axis cs:-0.025,0) rectangle (axis cs:0.025,0.39);
\draw[draw=none,fill=darkorange25512714] (axis cs:0.025,0) rectangle (axis cs:0.075,0.22);
\draw[draw=none,fill=forestgreen4416044] (axis cs:0.075,0) rectangle (axis cs:0.125,0.13);
\addplot [semithick, black, dash pattern=on 1pt off 3pt on 3pt off 3pt]
table {%
-0.0325000000000002 0.07
0.1325 0.07
};
\addplot [semithick, red, dashed]
table {%
-0.0325000000000002 0.41
0.1325 0.41
};
\end{groupplot}

\end{tikzpicture}

==> prompts/ALFworld/primitives.tex <==
\begin{mdframed}[style=mystyle, frametitle={ALFworld: Distilled orimitives only knowledge}]
\addcontentsline{toc}{paragraph}{ALFworld: Distilled orimitives only knowledge}
\small\ttfamily
\begin{spverbatim}
Please only generate following actions in your response:

    go to [receptacle] [id]
    # Example: 
        go to countertop 1
    take [object] [id] from [receptacle] [id]
    # Example:
        take mug 1 from countertop 1
    put [object] [id] in/on [receptacle] [id]
    # Example: 
        put laptop 1 in/on ottoman 1
    clean [object] [id] with [receptacle] [id]
    # Example: 
        clean ladle 2 with sinkbasin 1
    open [object] [id]
    # Example: 
        open cabinet 9
    use [object] [id]
    # Example: 
        use desklamp 1
    heat [object] [id] with [receptacle] [id]
    # Example: 
        heat egg 1 with microwave 1
    cool [object] [id] with [receptacle] [id]
    # Example: 
        cool lettuce 3 with fridge 1
\end{spverbatim}
\end{mdframed}

==> prompts/Webshop/primitives_only.tex <==
\begin{mdframed}[style=mystyle, frametitle={Webshop: Distilled primitives only knowledge prompt}]
\addcontentsline{toc}{paragraph}{Webshop: Distilled primitives only knowledge prompt}
\small\ttfamily
\begin{spverbatim}
Please only generate following actions in your response:

    search[Query]
    # Example search[3 ounce bright citrus deodorant sensitive skin]
    click[Product ID]
    # Example click[B0054KM7IY]
    click[Size]
    # Example click[38 m eu]
    click[Color]
    # Example click[brown]
    click[Buy Now]
    click[Style]
    # Example click[powerlite 1785w]
    click[< Prev]
    click[Flavor]
    # Example click[plantain chips]
    click[Features]
    # Example click[Features]
    click[Shape]
    # Example click[rectangular]
    click[Description]
    # Example click[Description]
    click[Offer Type]
    # Example click[lockscreen ad-supported]
    click[Digital Storage Capacity]
    # Example click[32 gb]
    click[Back to Search]
    click[Fit Type]
    # Example click[men]
\end{spverbatim}
\end{mdframed}

==> table_tips_alfworld.tex <==
\begin{table}
\caption {Results in ALFWorld}
\begin{tabular}{c|c}
\toprule
Method & Tips \\
\cmidrule{1-2}
LLM-generated & 1. Use the correct preposition when placing an object on a surface. The correct action is to put the object "in/on" the surface, not just "on" the surface. \\ 2. Place the object in the first available and suitable location instead of unnecessarily checking other locations. \\ 3. If you put an object in a device (like a microwave), remember to take it out before trying to put it in another location.
\bottomrule
\end{tabular}
\end{table}

==> tables_1.tex <==
\definecolor{LightCyan}{rgb}{0.88,1,1}
\begin{table*}
\centering
\resizebox{0.95\textwidth}{!}{
% \captionsetup{justification=centering}
% \caption {Results of \llmpolname and \codepolname in ALFworld}
% \label{table:majorresults}
\begin{minipage}[t]{0.61\textwidth}
\caption {Results in ALFWorld}
\vspace{-1em}
\label{main_results_alfworld}
\resizebox{1.05\textwidth}{!}{
\begin{tabular}{c|c|cccccc|c}
\toprule
Model  & Method & Pick & Clean & Heat & Cool & Look & Pick2 & All \\
\midrule
% \multicolumn{9}{c}{Text-based Policy} \\
% \cmidrule{1-9}
\multirow{ 2}{*}{\shortstack{GPT-4\\(0613)}} & ReAct    & 67 & 74 & 74 & 67 & 100 & 47 & 72\\
                            & \ourmod   & \bf{92} & \bf{100} & \bf{96} & \bf{95} & \bf{100} & \bf{53} & \bf{91}\\
                            % &\rowcolor{LightCyan}\ourmod\texttt{-Human} & 83 & 100 & 87 & 95 & 100 & 53 & 88\\
\cmidrule{1-9}
\multirow{ 2}{*}{\shortstack{GPT-3.5\\(0613)}} & ReAct  & 13  & 10  & 0  &  0 & 17 & 0 & 7\\
                            & \ourmod       & \bf{71} & \bf{35} & \bf{4}  & \bf{67} & \bf{44} & \bf{24} & \bf{41}\\
                         % & \rowcolor{LightCyan}\ourmod\texttt{-Human} & 71 & 68 & 83 & 71 & 44 & 24 & 63\\
% \cmidrule{1-9}
% \multicolumn{9}{c}{Code-based Policy} \\
% \cmidrule{1-9}
% \multirow{ 2}{*}{\shortstack{GPT-4\\(0613)}} & Demo2Code    & 96       & 58      & 13      & 43      & 0       & 65      & 48\\
%                                              & \ourmodcode  & \bf{100} & \bf{84} & \bf{87} & \bf{90} & \bf{89} & \bf{88} & \bf{90}\\
% \cmidrule{1-9}
% \multirow{ 2}{*}{\shortstack{GPT-3.5\\(0613)}} & Demo2Code & 96        & 26      & 48      & 29      & 0       & \bf{82} & 46\\
%                                & \ourmodcode               & \bf{100}  & \bf{71} & \bf{91} & \bf{86} & \bf{89} & 18 & \bf{78}\\
\bottomrule
\end{tabular}
}
\end{minipage}
\hspace{5mm}
\vline
\hspace{1mm}
\begin{minipage}[t]{0.3\textwidth}
\caption {Results in WebShop}
\vspace{-0.95em}
\label{main_results_webshop}
% \begin{wraptable}{r}{6.6cm}
% \begin{table}
% \captionsetup{justification=centering}
% \caption {Results of \llmpolname and \codepolname in Webshop}
% \label{table:majorresults}
% \centering
\resizebox{1.105\textwidth}{!}{
\begin{tabular}{c|c|c|c}
\toprule
Model  & Method & SR & Score \\
\midrule
% \multicolumn{4}{c}{Text-based Policy} \\
% \cmidrule{1-4}
\multirow{ 2}{*}{\shortstack{GPT-4\\(0613)}} & ReAct & 26 & 39 \\
                            & \ourmod& \bf{41} & \bf{58}\\
                            % & \rowcolor{LightCyan}\ourmodhuman& 41 & 61\\
\cmidrule{1-4}
\multirow{ 2}{*}{\shortstack{GPT-3.5\\(0613)}} & ReAct & 27 & 60\\
                            & \ourmod                & \bf{35} & \bf{61}\\
                            % & \rowcolor{LightCyan}\ourmodhuman           & 31      & 61 \\
% \cmidrule{1-4}
% \multirow{ 3}{*}{\shortstack{GPT-3.5\\(0301)}} & ReAct & 12 & 28\\
%                             & \ourmod                  & \bf{18} & \bf{33}\\
%                             & \rowcolor{LightCyan}\ourmodhuman             & 20 & 35 \\
% \cmidrule{1-4}
% \multicolumn{4}{c}{Code-based Policy} \\
% \cmidrule{1-4}
% \multirow{ 2}{*}{\shortstack{GPT-4\\(0613)}} & Demo2Code & 1 & 5\\
%                             & \ourmodcode & \bf{19} & \bf{31}\\
% \cmidrule{1-4}
% \multirow{ 2}{*}{\shortstack{GPT-3.5\\(0613)}} & Demo2Code & 0 & 0\\
%                                & \ourmodcode & 0 & 0\\
\bottomrule
\end{tabular}
% \end{wraptable}
}
\end{minipage}
}
\end{table*}




